An APTAS for Bin Packing with Clique-graph Conflicts

We study the following variant of the classic {\em bin packing} problem. Given a set of items of various sizes, partitioned into groups, find a packing of the items in a minimum number of identical (unit-size) bins, such that no two items of the same group are assigned to the same bin. This problem, known as {\em bin packing with clique-graph conflicts}, has natural applications in storing file replicas, security in cloud computing and signal distribution. Our main result is an {\em asymptotic polynomial time approximation scheme (APTAS)} for the problem, improving upon the best known ratio of $2$. %In particular, for any instance $I$ and a fixed $\eps \in (0,1)$, the items are packed in at most $(1+\eps)OPT(I) +1$ bins, where $OPT(I)$ is the minimum number of bins required for packing the instance. As a key tool, we apply a novel {\em Shift \& Swap} technique which generalizes the classic linear shifting technique to scenarios allowing conflicts between items. The major challenge of packing {\em small} items using only a small number of extra bins is tackled through an intricate combination of enumeration and a greedy-based approach that utilizes the rounded solution of a {\em linear program}.

==> discussion.tex <==

\section{Discussion}\label{Discussion}
\label{sec:Discussion}

In Section~\ref{sec:APTAS} we construct an APTAS for GBP, thus improving the best known approximation ratio of 2 \cite{allornothing} by almost twofold. Until now, only restricted GBP instances, for which the groups contain a constant number of items, had an asymptotic approximation scheme. This is due to an AFPTAS for BP with d-inductive conflict graph, where $d$ is a constant \cite{jansen1999approximation}. The question of whether GBP admits an APTAS for groups of unbounded size was brought to light by McCloskey and Shankar \cite{mccloskey2005approaches}, and henceforth, it is resolved by the results of this paper. Moreover, this paper achieves a better constant, $1$, in comparison to the constant of $\frac{d}{\eps^2}$ for d-inductive graphs \cite{jansen1999approximation}. Namely, our constant does not depend on $\eps$ nor on the size of the maximal group.  

A variety of techniques are integrated in this scheme, including enhancement of linear shifting and a complex greedy-based approach for packing the small items. We generalize the scheme for bin packing with {\em proper interval} conflict graphs and {\em constant length interval} conflict graphs in~\cite{CITEOURPAPER}. It would be interesting to find APTAS for bin packing with other families of conflict graphs using similar techniques. The techniques proposed in this paper are tailored for bin packing with conflicts. However, some of the techniques may be useful for other resource allocation problems with conflicting items.





